A survey on power maps in groups

The study of word maps on groups has been of deep interest in recent years. This survey focuses on the case of power maps on groups; $viz.$ the map $x\mapsto x^M$ for a group $G$, and an integer $M\geq 2$. Here, we accumulate various results on the subject and pose some questions.

==> extra-conj-cent.tex <==
\subsection{General linear group} Given a $n$-dimensional vector space $V$ over $\fq$, the set of all automorphisms of $V$ is denoted by $\GL(V)$ and after
fixing an appropriate basis, $\GL(V)$ can be identified with $\GL_n(q)$. 
The conjugacy classes of $\GL_n(q)$ are determined by functions 
$\lambda:\Phi\longrightarrow\Lambda$ by $f\mapsto\lambda_f$ such that $\sum\limits_{f}\deg(f)\cdot|\lambda_f|=n$. The combinatorial data $\{(f,\lambda_f):f\in\Phi\}$ attached via this correspondence, for an element $\alpha\in \GL_n(q)$ will be denoted by $\Delta(\alpha)$. The centralizer size 
is given by
\begin{align*}
    \prod\limits_{\varphi\in\Delta(\alpha)}\left(q^{\deg \varphi\cdot \sum\limits_{i}(\lambda_{i,\varphi}')^2}\prod_{i\geq 1}\left(\dfrac{1}{q^{\deg\varphi}}\right)_{m_i(\lambda_\varphi)}\right).
\end{align*}
\subsection{Symplectic and orthogonal groups}\label{subsec:symporth}
First, fix the matrix
\begin{equation}\label{def:pi-n}
\Pi_n=\begin{pmatrix} 0 & 0 & \cdots & 0 & 1\\
0 & 0 & \cdots & 1 & 0\\ \vdots & \vdots & \reflectbox{$\ddots$} & \vdots & \vdots\\
1 & 0 & \cdots & 0 & 0 \end{pmatrix}.    
\end{equation}
\subsubsection{Symplectic group}
Let $V$ be a vector space of dimension $2n$ over $\mathbb F_q$. There is a unique non-degenerate alternating bilinear form on $V$. We consider the form given by 
$$\left<(x_i)_{i=1}^{2n}, (y_j)_{j=1}^{2n} \right> = \sum_{j=1}^{n}x_jy_{2n+1-j}-\sum_{i=0 } ^{n-1}x_{2n-i}y_{i+1}.$$ 
The symplectic group is the subgroup of $\GL(V)$ consisting of those elements which preserve this alternating form on $V$. 
By fixing an appropriate basis, the matrix of the form is $J= \begin{pmatrix} 0 & \Pi_n\\ -\Pi_n & 0 \end{pmatrix}$ where  
$$\SP_{2n}(q)=\{A \in \GL_{2n}(q) \mid \tr AJA=J\}.$$ 
Since all non-degenerate alternating forms are equivalent over $\mathbb F_q$, the symplectic groups obtained with respect to different forms are conjugate within $\GL_{2n}( q)$. 
\subsubsection{Orthgonal Groups}
Let $V$ be an $m$-dimensional vector space over a finite field $\mathbb F_q$. Then there are at most two non-equivalent non-degenerate quadratic forms on $V$. The orthogonal group consists of elements of $\GL(V)$ which preserve a non-degenerate quadratic form $Q$. 

When $m=2n$ for some $n\geq 1$, up to equivalence there are two such forms denoted as $Q^+$ and $Q^-$. These are as follows. Fix $a\in \mathbb F_q$ such that $t^2 + t + a \in \fq[t]$ is irreducible. Then the two non-equivalent forms are given by
\begin{enumerate}
\item $Q^+(x_1, \ldots, x_m) = x_{1}x_{2} + x_3x_4+\cdots + x_{2n-1}x_{2n}$, and
\item $Q^-(x_1,\ldots, x_m)= x_1^2 + x_1x_2+ax_2^2 + x_3x_4+\cdots + x_{2n-1}x_{2n}$.
\end{enumerate}
The orthogonal group preserving $Q^+$ will be denoted as $\On{+}_m(q)$, and the orthogonal group preserving $Q^-$ will be denoted as $\On{-}_m(q)$. For odd $m$ up to equivalence, there are two non-degenerate quadratic forms. But, these two forms give isomorphic orthogonal groups. We take $Q(x_1, \ldots, x_m)= x_1^2+\cdots + x_m^2$. Thus, in case $m=2n+1$, up to conjugacy, we have only one orthogonal group. This will be denoted as $\On{}(m, q)$. 

As is common in the literature, we will use the notation $\On{\epsilon}_m(q)$ to denote any of the orthogonal group above where $\epsilon \in \{~, +, -\}$. With respect to an appropriate basis, we will fix the matrices of the symmetric bilinear forms (associated to the quadratic forms $Q^{\epsilon}$) as follows: 
$$J_{0}=\begin{pmatrix} 0 & 0 & \Pi_n \\ 0 & \alpha & 0\\ \Pi_n & 0 & 0 
\end{pmatrix},  J_{+}=\begin{pmatrix} 0& \Pi_n\\ \Pi_n & 0
\end{pmatrix}, J_{-}=\begin{pmatrix} 0 & 0 & 0 & \Pi_{n-1}\\
0 & 1 & 0 & 0 \\ 0 & 0 & -\delta & 0 \\ \Pi_{n-1}& 0 & 0 & 0
\end{pmatrix}$$ 
where $\alpha\in\fq^\times,\delta\in\fq\setminus\fq^2$ and $\Pi_n$ as in \cref{def:pi-n}.
Then, the orthogonal group in matrix form is 
$$\On{\e}_m( q) = \{A \in \GL_m(q)\mid \tr{A}J_{\e}A=J_{\e}\}.$$

% Adapting the notations of \cite{FuNePr05book}, we define the type of an orthogonal space as follows.

% \emph{The type of an orthogonal space} $(V,Q)$ of dimension $m$ is
% \begin{align*}
% \tau(V)=\begin{cases}
% 1 & \text{if } m \text{ is odd, }q\equiv 1\imod 4, Q\sim\sum x_i^2,\\
% -1 & \text{if } m \text{ is odd, }q \equiv 1\imod 4, Q\sim b\sum x_i^2,\\
% \iota^m & \text{if } m \text{ is odd, }q\equiv 3\imod 4, Q\sim\sum x_i^2,\\
% (-\iota)^m & \text{if } m \text{ is odd, }q\equiv 3\imod 4, Q\sim b\sum x_i^2,
% \end{cases}
% \end{align*}
% where $\iota\in\mathbb{C}$ satisfies $\iota^2=-1$, and $b\in\fq\setminus\fq^2$.
%  More generally, when $V$ is orthogonal direct sum $V_1\oplus V_2 \oplus \cdots \oplus V_l$, the type is defined by $\tau(V)=\prod\limits_{i=1}^l\tau(V_i)$.

% %%%%%%%%%%%%

Now we describe the conjugacy classes and the centralizer of an element in 
finite symplectic and orthogonal groups. 
This is given in \cite{wall63}. 
We recall briefly the results therein, which will be used further.
A \textbf{symplectic signed partition} is a partition of a number $k$, such that each odd part has an even multiplicity and each even part has a sign associated with it. 
The set of all symplectic signed partitions will be denoted as $\ssp_{\Sp}$.
An \textbf{orthogonal signed partition} is a partition of a number $k$, such that each even part has an even multiplicity, and each odd part has a sign associated with it. 
The set of all orthogonal signed partitions will be denoted as $\ssp_{\On{}}$.
The \textit{dual} of a monic degree $r$ polynomial $f(x)\in k[x]$ satisfying $f(0)\neq 0$, is the polynomial given by $f^*(x)=f(0)^{-1}x^rf(x^{-1})$. 
A \emph{self reciprocal irreducible monic} (SRIM) polynomial is a monic irreducible polynomial satisfying $f=f^*$.

% The polynomial $f$ will be called \textit{$*$-symmetric} (or \emph{self reciprocal}) if $f=f^*$. A monic polynomial $f(x)\in \fq[x]$, will be called to be \textbf{$*-$irreducible}
%  if and only if it does not have any proper self-reciprocal factor.
% It can be shown that the characteristic polynomial of a symplectic or orthogonal matrix is self-reciprocal. Indeed if $\mu$ is a root of the characteristic 
% polynomial of a symplectic (or orthogonal) matrix, so is $\mu^{-1}$. We follow 
% J. Milnor's terminology \cite{milnor69} to distinguish between the $*$-irreducible factors of the characteristic polynomials. We call a $*$-irreducible polynomial $f$ to be
% (1) Type $1$\index{Type $1$ polynomial} if $f=f^*$ and $f$ is irreducible polynomial of even degree;
% (2) Type $2$\index{Type $2$ polynomial} if $f=gg^*$ and $g$ is irreducible polynomial satisfying $g\neq g^*$;
% (3) Type $3$\index{Type $3$ polynomial} if $f(x)=x\pm 1$.

According to \cite{wall63}, \cite{shinoda80}, the conjugacy classes of $\Sp_{2n}(q)$ are parameterized by the functions 
$\lambda:\Phi\rightarrow\pa^{2n}\cup\ssp_{\Sp}^{2n}$, where $\Phi$ denotes the set of all
 monic,  non-constant, irreducible polynomials, $\pa^{2n}$ is
 the set of all partitions 
of $1\leq k\leq 2n$ and $\ssp_{\Sp}^{2n}$ is the set of all symplectic
 signed partitions 
of $1\leq k\leq 2n$. Such a $\lambda$ represents a conjugacy class of $\Sp_{2n}(q)$
if and only if  (a) $\lambda(u)=0$, (b)
 $\lambda_{\varphi^*}=\lambda_\varphi$, (c)
 $\lambda_\varphi\in\ssp^n_{\Sp}$ iff $\varphi=u\pm 1$ (we distinguish this $\lambda$, by denoting it $\lambda^\pm$) and, (d)
 $\displaystyle\sum_{\varphi}|\lambda_\varphi|\textup{deg}(\varphi)=2n$.
Also from \cite{wall63}, \cite{shinoda80}, we find that a similar kind of statement is true for the groups $\On{\epsilon}_n(q)$. The conjugacy classes of $\On{\epsilon}_n(q)$ are parameterized by the functions 
$\lambda:\Phi\rightarrow\pa^{n}\cup\ssp_{\On{}{}}^{n}$, where $\Phi$ denotes the set of all
 monic,  non-constant, irreducible polynomials, $\pa^{n}$ is
 the set of all partitions 
of $1\leq k\leq n$ and $\ssp_{\On{}}^{n}$ is the set of all symplectic
 signed partitions 
of $1\leq k\leq n$. Such a $\lambda$ represents a conjugacy class of $\On{\epsilon}_{n}(q)$ for $\epsilon=\pm$,
if and only if (a)
 $\lambda(x)=0$, (b)
 $\lambda_{\varphi^*}=\lambda_\varphi$, (c)
 $\lambda_\varphi\in\ssp^n_{\On{}}$ iff $\varphi=u\pm 1$ (we distinguish this $\lambda$, by denoting it $\lambda^\pm$) and, (d)
 $\displaystyle\sum_{\varphi}|\lambda_\varphi|\textup{deg}(\varphi)=n$.
Class representative corresponding to given data can be found in \cite{ta1}, \cite{ta2}, \cite{glo} 
and we will mention them whenever needed. The results about the conjugacy class size (and hence the size of the centraliser)
 of elements corresponding to given data can be found in \cite{wall63}.
% \begin{lemma}\cite[pp. 36]{wall63}\label{lem:centralizer-sizes-symp}
% Let $X\in\Sp_{2n}(q)$ be a matrix corresponding to the data $\Delta(X)=\{(\varphi,\mu_\varphi)
% :\varphi\in\Phi\}$. Then the conjugacy class of
% $X$ in $\Sp_{2n}(q)$ is of size $\dfrac{|\Sp_{2n}(q)|}{\prod\limits_{\varphi}B(\varphi)}$
% where $B(\varphi)$ and $A(\varphi^\mu)$ are defined as follows
% \begin{align*}
% A(\varphi^\mu)=\begin{cases}
% |\U_{m_\mu}(Q)| & \text{if } \varphi(x)=\varphi^*(x)\neq x\pm 1\\
% |\GL_{m_\mu}(Q)|^\frac{1}{2}& \text{if } \varphi\neq\varphi^*\\
% |\Sp_{m_\mu}(q)| &\text{if }\varphi(x)=x\pm 1,~\mu\text{ odd}\\
% |q^{\frac{1}{2}m_\mu}\On{\epsilon}_{m_\mu}(q)|&\text{if }\varphi(x)=x\pm 1,~\mu\text{ even}
% \end{cases}
% \end{align*}
% where $\e$ gets determined by the sign of the corresponding partition, 
% $Q=q^{|\varphi|}$, $m_\mu=m(\varphi^\mu)$ and
% \begin{align*}
% B(\varphi) = Q^{\sum\limits_{\mu<\nu}\mu m_\mu m_\nu+
% \frac{1}{2}\sum\limits_{\mu}(\mu-1)m_\mu^2}\prod\limits_{\mu}A(\varphi^\mu).
% \end{align*}
% \end{lemma}
% \begin{lemma}\cite[pp. 39]{wall63}\label{centra-size-on}
% Let $X\in\On{\e}_n(q)$ be a matrix corresponding to the data $\Delta(X)=\{(\varphi,\mu_\varphi)
% :\varphi\in \Phi\}$. Then the conjugacy class of
% $X$ in $\On{\e}_n(q)$ is of size $\dfrac{|\On{\e}_n(q)|}{\prod\limits_{\varphi}B(\varphi)}$
% where $B(\varphi)$ and $A(\varphi^\mu)$ are defined as before, except when $\varphi(x)=x\pm 1$,
% \begin{align*}
% A(\varphi^\mu)=\begin{cases}
% |\On{\epsilon'}_{m_\mu}(q)|&\text{if }\mu\text{ odd}\\
% q^{-\frac{1}{2}m_{\mu}}|\Sp_{m_\mu}(q)|&\text{if }\mu\text{ even}
% \end{cases}
% \end{align*}
% where $\e'$ in $\On{\e'}_{m_\mu}(q)$  gets determined by the 
% corresponding sign of the part, of the partition.
% \end{lemma}
% {\color{blue}The quantity $B(\varphi)$ will also be denoted as $c_{\Sp,\varphi,q}(\lambda^{\pm})$ in case of symplectic groups and as $c_{\On{\epsilon},\varphi, q}(\lambda^\pm)$ in case of orthogonal groups when $\varphi=x\pm 1$.}
\subsection{Unitary groups}
Consider the field $k=\mathbb F_{q^2}$, and the involution $\sigma \colon \fqn{2}\longrightarrow\fqn{2}$ defined as $\sigma(a):=\overline{a}=a^q$ of the field. We further get an automorphism of
$\fqn{2}[t]$, the polynomial ring over $\fqn{2}$, by action on the coefficients of the polynomials. The image of
$f\in\fqn{2}[t]$ will be denoted as $\overline{f}$. Consider the Hermitian form given by the matrix
$
\Pi_n$.
Then we identify the unitary group (corresponding to the above Hermitian form) with the set
\[
\U_n(\fqn{2})=\left\{A\in\GL_n(\fqn{2})\mid  A\Pi_n\overline{A}^t=\Pi_n\right\}.
\]
Since all non-degenerate Hermitian forms on an $n$-dimensional vector space are unitarily congruent to the Hermitian form given by the above matrix,
it is evident that all the unitary groups arising are conjugate with each other inside
$\GL_n(q^2)$ (see theorem $10.3$ of \cite{Gr02}). From the work of Wall, it is known that two elements $g_1, g_2 \in\U_n(q^2)$ are conjugate to each other if and only if they are conjugate in $\GL_n(q^2)$.
These conjugacy classes are parameterized by special polynomials and partitions.
A \emph{$\sim$-symmetric} or \emph{self conjugate} polynomial is a polynomial $f$ of degree $d$ such that $\widetilde{f}=f$ where $\widetilde{f}(t) = \overline{f(0)}^{-1} t^d \bar f(t^{-1})$. A polynomial without a proper $\sim$-symmetric factor is referred to as a \emph{$\sim$-irrdeucible} polynomial. Note that a $\sim$-irreducible polynomial can be reducible in the usual sense.
Denote by $\widetilde{\Phi}$ to be the set of all $\sim$-irreducible polynomials. 
 Then a conjugacy class in $\U(n,\fqn{2})$ is determined by a function $\lambda\colon \widetilde{\Phi} \longrightarrow \Lambda$ which satisfies
(a) $\lambda(f)=\lambda(\widetilde{f})$ and, (b) $\sum\limits_{\varphi}|\lambda(\varphi)|\deg\varphi=n$. The centralizer size can be found in \cite{wall63} and we are not quoting it here.

Using this information,
we determine when a matrix $A$ has an $M$-th root in the given group $G_n(q)$. 
This information is further used to determine the 
desired generating functions, with the help of the concept of 
the central join of two matrices, following \cite{ta1}, \cite{ta2}, \cite{ta3}.
\color{black}
%%%%%(x + 1) * (x + 2) * (x + a) * (x + a + 1) * (x + a + 2) * (x + 2*a) * (x + 2*a + 1) * (x + 2*a + 2) * (x^3 + x + a) * (x^3 + x + a + 1) * (x^3 + x + a + 2) * (x^3 + x + 2*a) * (x^3 + x + 2*a + 1) * (x^3 + x + 2*a + 2) * (x^3 + 2*x + 1) * (x^3 + 2*x + 2) * (x^3 + 2*x + a) * (x^3 + 2*x + a + 2) * (x^3 + 2*x + 2*a) * (x^3 + 2*x + 2*a + 1) * (x^3 + (a + 1)*x + 1) * (x^3 + (a + 1)*x + 2) * (x^3 + (a + 1)*x + a) * (x^3 + (a + 1)*x + a + 1) * (x^3 + (a + 1)*x + 2*a) * (x^3 + (a + 1)*x + 2*a + 2) * (x^3 + (2*a + 2)*x + 1) * (x^3 + (2*a + 2)*x + 2) * (x^3 + (2*a + 2)*x + a + 1) * (x^3 + (2*a + 2)*x + a + 2) * (x^3 + (2*a + 2)*x + 2*a + 1) * (x^3 + (2*a + 2)*x + 2*a + 2) * (x^3 + x^2 + 2) * (x^3 + x^2 + a + 1) * (x^3 + x^2 + 2*a + 2) * (x^3 + x^2 + x + 2) * (x^3 + x^2 + x + a + 1) * (x^3 + x^2 + x + 2*a + 2) * (x^3 + x^2 + 2*x + 1) * (x^3 + x^2 + 2*x + a) * (x^3 + x^2 + 2*x + 2*a + 1) * (x^3 + x^2 + a*x + 1) * (x^3 + x^2 + a*x + a + 2) * (x^3 + x^2 + a*x + 2*a + 2) * (x^3 + x^2 + (a + 1)*x + 2) * (x^3 + x^2 + (a + 1)*x + a + 2) * (x^3 + x^2 + (a + 1)*x + 2*a + 1) * (x^3 + x^2 + (a + 2)*x + 1) * (x^3 + x^2 + (a + 2)*x + a) * (x^3 + x^2 + (a + 2)*x + 2*a + 1) * (x^3 + x^2 + 2*a*x + 1) * (x^3 + x^2 + 2*a*x + a) * (x^3 + x^2 + 2*a*x + 2*a + 1) * (x^3 + x^2 + (2*a + 1)*x + 1) * (x^3 + x^2 + (2*a + 1)*x + a + 1) * (x^3 + x^2 + (2*a + 1)*x + 2*a) * (x^3 + x^2 + (2*a + 2)*x + 2) * (x^3 + x^2 + (2*a + 2)*x + a) * (x^3 + x^2 + (2*a + 2)*x + 2*a) * (x^3 + 2*x^2 + 1) * (x^3 + 2*x^2 + a + 1) * (x^3 + 2*x^2 + 2*a + 2) * (x^3 + 2*x^2 + x + 1) * (x^3 + 2*x^2 + x + a + 1) * (x^3 + 2*x^2 + x + 2*a + 2) * (x^3 + 2*x^2 + 2*x + 2) * (x^3 + 2*x^2 + 2*x + a + 2) * (x^3 + 2*x^2 + 2*x + 2*a) * (x^3 + 2*x^2 + a*x + 2) * (x^3 + 2*x^2 + a*x + a + 1) * (x^3 + 2*x^2 + a*x + 2*a + 1) * (x^3 + 2*x^2 + (a + 1)*x + 1) * (x^3 + 2*x^2 + (a + 1)*x + a + 2) * (x^3 + 2*x^2 + (a + 1)*x + 2*a + 1) * (x^3 + 2*x^2 + (a + 2)*x + 2) * (x^3 + 2*x^2 + (a + 2)*x + a + 2) * (x^3 + 2*x^2 + (a + 2)*x + 2*a) * (x^3 + 2*x^2 + 2*a*x + 2) * (x^3 + 2*x^2 + 2*a*x + a + 2) * (x^3 + 2*x^2 + 2*a*x + 2*a) * (x^3 + 2*x^2 + (2*a + 1)*x + 2) * (x^3 + 2*x^2 + (2*a + 1)*x + a) * (x^3 + 2*x^2 + (2*a + 1)*x + 2*a + 2) * (x^3 + 2*x^2 + (2*a + 2)*x + 1) * (x^3 + 2*x^2 + (2*a + 2)*x + a) * (x^3 + 2*x^2 + (2*a + 2)*x + 2*a) * (x^3 + a*x^2 + a) * (x^3 + a*x^2 + a + 2) * (x^3 + a*x^2 + 2*a) * (x^3 + a*x^2 + x + 1) * (x^3 + a*x^2 + x + 2) * (x^3 + a*x^2 + x + a + 2) * (x^3 + a*x^2 + 2*x + a + 1) * (x^3 + a*x^2 + 2*x + a + 2) * (x^3 + a*x^2 + 2*x + 2*a + 2) * (x^3 + a*x^2 + a*x + 2) * (x^3 + a*x^2 + a*x + 2*a + 1) * (x^3 + a*x^2 + a*x + 2*a + 2) * (x^3 + a*x^2 + (a + 1)*x + a) * (x^3 + a*x^2 + (a + 1)*x + a + 2) * (x^3 + a*x^2 + (a + 1)*x + 2*a) * (x^3 + a*x^2 + (a + 2)*x + 2) * (x^3 + a*x^2 + (a + 2)*x + 2*a + 1) * (x^3 + a*x^2 + (a + 2)*x + 2*a + 2) * (x^3 + a*x^2 + 2*a*x + 1) * (x^3 + a*x^2 + 2*a*x + 2*a) * (x^3 + a*x^2 + 2*a*x + 2*a + 1) * (x^3 + a*x^2 + (2*a + 1)*x + a) * (x^3 + a*x^2 + (2*a + 1)*x + a + 1) * (x^3 + a*x^2 + (2*a + 1)*x + 2*a + 1) * (x^3 + a*x^2 + (2*a + 2)*x + 2) * (x^3 + a*x^2 + (2*a + 2)*x + 2*a + 1) * (x^3 + a*x^2 + (2*a + 2)*x + 2*a + 2) * (x^3 + (a + 1)*x^2 + 1) * (x^3 + (a + 1)*x^2 + 2) * (x^3 + (a + 1)*x^2 + a + 1) * (x^3 + (a + 1)*x^2 + x + a) * (x^3 + (a + 1)*x^2 + x + a + 2) * (x^3 + (a + 1)*x^2 + x + 2*a + 2) * (x^3 + (a + 1)*x^2 + 2*x + 1) * (x^3 + (a + 1)*x^2 + 2*x + 2) * (x^3 + (a + 1)*x^2 + 2*x + a + 1) * (x^3 + (a + 1)*x^2 + a*x + a) * (x^3 + (a + 1)*x^2 + a*x + a + 2) * (x^3 + (a + 1)*x^2 + a*x + 2*a + 2) * (x^3 + (a + 1)*x^2 + (a + 1)*x + a + 1) * (x^3 + (a + 1)*x^2 + (a + 1)*x + a + 2) * (x^3 + (a + 1)*x^2 + (a + 1)*x + 2*a + 1) * (x^3 + (a + 1)*x^2 + (a + 2)*x + 1) * (x^3 + (a + 1)*x^2 + (a + 2)*x + 2*a + 1) * (x^3 + (a + 1)*x^2 + (a + 2)*x + 2*a + 2) * (x^3 + (a + 1)*x^2 + 2*a*x + 2) * (x^3 + (a + 1)*x^2 + 2*a*x + 2*a) * (x^3 + (a + 1)*x^2 + 2*a*x + 2*a + 2) * (x^3 + (a + 1)*x^2 + (2*a + 1)*x + a) * (x^3 + (a + 1)*x^2 + (2*a + 1)*x + a + 2) * (x^3 + (a + 1)*x^2 + (2*a + 1)*x + 2*a + 2) * (x^3 + (a + 1)*x^2 + (2*a + 2)*x + a) * (x^3 + (a + 1)*x^2 + (2*a + 2)*x + a + 1) * (x^3 + (a + 1)*x^2 + (2*a + 2)*x + 2*a) * (x^3 + (a + 2)*x^2 + a) * (x^3 + (a + 2)*x^2 + a + 2) * (x^3 + (a + 2)*x^2 + 2*a + 1) * (x^3 + (a + 2)*x^2 + x + 1) * (x^3 + (a + 2)*x^2 + x + 2) * (x^3 + (a + 2)*x^2 + x + a) * (x^3 + (a + 2)*x^2 + 2*x + a) * (x^3 + (a + 2)*x^2 + 2*x + a + 1) * (x^3 + (a + 2)*x^2 + 2*x + 2*a + 2) * (x^3 + (a + 2)*x^2 + a*x + a + 1) * (x^3 + (a + 2)*x^2 + a*x + a + 2) * (x^3 + (a + 2)*x^2 + a*x + 2*a) * (x^3 + (a + 2)*x^2 + (a + 1)*x + 1) * (x^3 + (a + 2)*x^2 + (a + 1)*x + 2*a) * (x^3 + (a + 2)*x^2 + (a + 1)*x + 2*a + 2) * (x^3 + (a + 2)*x^2 + (a + 2)*x + 2) * (x^3 + (a + 2)*x^2 + (a + 2)*x + 2*a) * (x^3 + (a + 2)*x^2 + (a + 2)*x + 2*a + 1) * (x^3 + (a + 2)*x^2 + 2*a*x + 1) * (x^3 + (a + 2)*x^2 + 2*a*x + 2*a) * (x^3 + (a + 2)*x^2 + 2*a*x + 2*a + 2) * (x^3 + (a + 2)*x^2 + (2*a + 1)*x + 1) * (x^3 + (a + 2)*x^2 + (2*a + 1)*x + 2*a) * (x^3 + (a + 2)*x^2 + (2*a + 1)*x + 2*a + 2) * (x^3 + (a + 2)*x^2 + (2*a + 2)*x + a) * (x^3 + (a + 2)*x^2 + (2*a + 2)*x + a + 2) * (x^3 + (a + 2)*x^2 + (2*a + 2)*x + 2*a + 1) * (x^3 + 2*a*x^2 + a) * (x^3 + 2*a*x^2 + 2*a) * (x^3 + 2*a*x^2 + 2*a + 1) * (x^3 + 2*a*x^2 + x + 1) * (x^3 + 2*a*x^2 + x + 2) * (x^3 + 2*a*x^2 + x + 2*a + 1) * (x^3 + 2*a*x^2 + 2*x + a + 1) * (x^3 + 2*a*x^2 + 2*x + 2*a + 1) * (x^3 + 2*a*x^2 + 2*x + 2*a + 2) * (x^3 + 2*a*x^2 + a*x + 1) * (x^3 + 2*a*x^2 + a*x + a + 1) * (x^3 + 2*a*x^2 + a*x + a + 2) * (x^3 + 2*a*x^2 + (a + 1)*x + a) * (x^3 + 2*a*x^2 + (a + 1)*x + 2*a) * (x^3 + 2*a*x^2 + (a + 1)*x + 2*a + 1) * (x^3 + 2*a*x^2 + (a + 2)*x + 1) * (x^3 + 2*a*x^2 + (a + 2)*x + a + 1) * (x^3 + 2*a*x^2 + (a + 2)*x + a + 2) * (x^3 + 2*a*x^2 + 2*a*x + 2) * (x^3 + 2*a*x^2 + 2*a*x + a) * (x^3 + 2*a*x^2 + 2*a*x + a + 2) * (x^3 + 2*a*x^2 + (2*a + 1)*x + a + 2) * (x^3 + 2*a*x^2 + (2*a + 1)*x + 2*a) * (x^3 + 2*a*x^2 + (2*a + 1)*x + 2*a + 2) * (x^3 + 2*a*x^2 + (2*a + 2)*x + 1) * (x^3 + 2*a*x^2 + (2*a + 2)*x + a + 1) * (x^3 + 2*a*x^2 + (2*a + 2)*x + a + 2) * (x^3 + (2*a + 1)*x^2 + a + 2) * (x^3 + (2*a + 1)*x^2 + 2*a) * (x^3 + (2*a + 1)*x^2 + 2*a + 1) * (x^3 + (2*a + 1)*x^2 + x + 1) * (x^3 + (2*a + 1)*x^2 + x + 2) * (x^3 + (2*a + 1)*x^2 + x + 2*a) * (x^3 + (2*a + 1)*x^2 + 2*x + a + 1) * (x^3 + (2*a + 1)*x^2 + 2*x + 2*a) * (x^3 + (2*a + 1)*x^2 + 2*x + 2*a + 2) * (x^3 + (2*a + 1)*x^2 + a*x + a) * (x^3 + (2*a + 1)*x^2 + a*x + 2*a + 1) * (x^3 + (2*a + 1)*x^2 + a*x + 2*a + 2) * (x^3 + (2*a + 1)*x^2 + (a + 1)*x + 2) * (x^3 + (2*a + 1)*x^2 + (a + 1)*x + a) * (x^3 + (2*a + 1)*x^2 + (a + 1)*x + a + 1) * (x^3 + (2*a + 1)*x^2 + (a + 2)*x + 1) * (x^3 + (2*a + 1)*x^2 + (a + 2)*x + a) * (x^3 + (2*a + 1)*x^2 + (a + 2)*x + a + 2) * (x^3 + (2*a + 1)*x^2 + 2*a*x + 2) * (x^3 + (2*a + 1)*x^2 + 2*a*x + a) * (x^3 + (2*a + 1)*x^2 + 2*a*x + a + 1) * (x^3 + (2*a + 1)*x^2 + (2*a + 1)*x + 2) * (x^3 + (2*a + 1)*x^2 + (2*a + 1)*x + a) * 
%(x^3 + (2*a + 1)*x^2 + (2*a + 1)*x + a + 1) * 
%(x^3 + (2*a + 1)*x^2 + (2*a + 2)*x + a + 2) * 
%(x^3 + (2*a + 1)*x^2 + (2*a + 2)*x + 2*a) * 
%(x^3 + (2*a + 1)*x^2 + (2*a + 2)*x + 2*a + 1) * 
%(x^3 + (2*a + 2)*x^2 + 1) * 
%(x^3 + (2*a + 2)*x^2 + 2) * 
%(x^3 + (2*a + 2)*x^2 + 2*a + 2) * 
%(x^3 + (2*a + 2)*x^2 + x + a + 1) * 
%(x^3 + (2*a + 2)*x^2 + x + 2*a) * 
%(x^3 + (2*a + 2)*x^2 + x + 2*a + 1) * 
%(x^3 + (2*a + 2)*x^2 + 2*x + 1) * 
%(x^3 + (2*a + 2)*x^2 + 2*x + 2) * 
%(x^3 + (2*a + 2)*x^2 + 2*x + 2*a + 2) * 
%(x^3 + (2*a + 2)*x^2 + a*x + a + 1) * 
%(x^3 + (2*a + 2)*x^2 + a*x + 2*a) * 
%(x^3 + (2*a + 2)*x^2 + a*x + 2*a + 1) * 
%(x^3 + (2*a + 2)*x^2 + (a + 1)*x + a + 2) * 
%(x^3 + (2*a + 2)*x^2 + (a + 1)*x + 2*a + 1) * 
%(x^3 + (2*a + 2)*x^2 + (a + 1)*x + 2*a + 2) * 
%(x^3 + (2*a + 2)*x^2 + (a + 2)*x + 2) * 
%(x^3 + (2*a + 2)*x^2 + (a + 2)*x + a + 1) * 
%(x^3 + (2*a + 2)*x^2 + (a + 2)*x + a + 2) * 
%(x^3 + (2*a + 2)*x^2 + 2*a*x + 1) * 
%(x^3 + (2*a + 2)*x^2 + 2*a*x + a) * 
%(x^3 + (2*a + 2)*x^2 + 2*a*x + a + 1) * 
%(x^3 + (2*a + 2)*x^2 + (2*a + 1)*x + a + 1) * 
%(x^3 + (2*a + 2)*x^2 + (2*a + 1)*x + 2*a) * 
%(x^3 + (2*a + 2)*x^2 + (2*a + 1)*x + 2*a + 1) * 
%(x^3 + (2*a + 2)*x^2 + (2*a + 2)*x + a) * %
%(x^3 + (2*a + 2)*x^2 + (2*a + 2)*x + 2*a) * 
%(x^3 + (2*a + 2)*x^2 + (2*a + 2)*x + 2*a + 2)
%%%%
